High-pressure TPCs in pressurized caverns: opportunities in dark matter and neutrino physics

The natural gas and hydrogen storage industries have experience creating huge, pressurized underground spaces. The most common of these is "solution mining", a method for making brine-filled cavities in salt formations. Unlike conventionally-mined underground spaces, these spaces are (a) inexpensive to construct and operate, (b) naturally serve as pressure vessels, at size scales impossible to construct in a conventional lab, and (b) permit safe use of flammable and/or toxic materials. If various engineering challenges could be met, solution-mined caverns would allow unprecedentedly-large high pressure gas TPCs. Lined rock caverns (LRC) may permit high pressure TPCs of considerable size in more conventional spaces. In this whitepaper, we review some of the new physics opportunities available in these caverns and suggest an R&D program needed to realize them.

==> table_0vbb.tex <==
  Target  & Endpoint & working point   &\multicolumn{2}{|c|}{m$_\nu$ = 50 meV} & m$_\nu$ giving \\ 
           &  keV     & P, T, $\rho$        &  Events/t/y & Events/m$^3$/y & 1 event/t/y \\ 
\hline 
H$_2$Se & 2998 & 9 bar, 273 K, 33.7 kg/m$^3$ & 22 & 0.7 & 10 meV \\ 
MoF$_6$ & 3035 & 1 bar, 320 K, 9.4 kg/m$^3$ & 26 & 0.2 & 9 meV \\ 
TeF$_6$ & 2527 & 10 bar, 273 K, 107.5 kg/m$^3$ & 3 & 0.4 & 27 meV \\ 
GeH$_4$ & 2039 & 50 bar, 273 K, 178.5 kg/m$^3$ & 1 & 0.3 & 36 meV \\ 
Xe & 2459 & 50 bar, 273 K, 303.4 kg/m$^3$ & 8 & 2.5 & 17 meV \\
